From Principles to Practice with Class in the First Year

We propose a bridge between functional and object-oriented programming in the first-year curriculum. Traditionally, curricula that begin with functional programming transition to a professional, usually object-oriented, language in the second course. This transition poses obstacles for students, and often results in confusing the details of development environments, syntax, and libraries with the fundamentals of OO programming that the course should focus on. Instead, we propose to begin the second course with a sequence of custom teaching languages which minimize the transition from the first course, and allow students to focus on core ideas. After working through the sequence of pedagogical languages, we then transition to Java, at which point students have a strong command of the basic principles. We have 3 years of experience with this course, with notable success.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Philip K.F. H\"olzenspies (Ed.): Trends on\\
Functional Programming In Education (TFPIE)\\
EPTCS 136, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.136.1}{10.4204/EPTCS.136.1}}

